Graph Topic Modeling for Documents with Spatial or Covariate Dependencies

We address the challenge of incorporating document-level metadata into topic modeling to improve topic mixture estimation. To overcome the computational complexity and lack of theoretical guarantees in existing Bayesian methods, we extend probabilistic latent semantic indexing (pLSI), a frequentist framework for topic modeling, by incorporating document-level covariates or known similarities between documents through a graph formalism. Modeling documents as nodes and edges denoting similarities, we propose a new estimator based on a fast graph-regularized iterative singular value decomposition (SVD) that encourages similar documents to share similar topic mixture proportions. We characterize the estimation error of our proposed method by deriving high-probability bounds and develop a specialized cross-validation method to optimize our regularization parameters. We validate our model through comprehensive experiments on synthetic datasets and three real-world corpora, demonstrating improved performance and faster inference compared to existing Bayesian methods.

==> 6.lit_review.tex <==

\paragraph{Bayesian approaches} Existing efforts to incorporate additional information into topic modeling have primarily worked with the Bayesian formulation of topic modeling, known as Latent Dirichlet Allocation (LDA) \citep{blei2001latent}. Traditional LDA frames the recovery of $W$ and $A$ as finding appropriate posteriors given the observed data $D$. In this setting, both $W$ and $A$ are considered to be random variables and endowed with prior probabilities, typically Dirichlet distributions. Letting $T_{im} \in \mathbb{R}^{p}$ be a one-hot vector representing the $m^{th}$ term of document $i$ (so that $D_{i\cdot} = \sum_{m=1}^{N_i}T_{im}$), the document corpus is assumed to be sampled from the following generative mechanism:
\begin{align}
 &\text{Topic Generation:}\notag\\
 &\qquad   \forall k \in [K], \qquad A_{k \cdot} \sim \text{Dirichlet}(\theta)\qquad  \text{ with  $\theta \in \R^{p}$ a hyperparameter} \tag{LDA 1}  \label{eq:dirichlet_samplingA}\\
  &\text{Document Generation:} \notag\\
  &\qquad   \forall i \in [n], \qquad W_{i \cdot} \sim \text{Dirichlet}(\alpha)\qquad  \text{ with  $\alpha \in \R^{K}$ a hyperparameter}\label{eq:dirichlet_samplingW}\tag{LDA 2} \\
  &\qquad   \forall m \in [N_i], \qquad Z_{im} \sim \text{Multinomial}(1, W_{i \cdot})\qquad  \text{(sampling of a topic for the $m^{th}$ word) } \notag\\
    &\qquad   \forall m \in [N_i], \qquad T_{im} \sim \text{Multinomial}(1, A_{Z_{im} \cdot})\qquad  \text{(sampling of a specific word) }  \tag{LDA 3} \label{eq:sampling}
\end{align}

%each topic $A_{k\cdot}$ is generated as: 
% \begin{equation}\label{eq:dirichlet_samplingA}
% A_{k \cdot} \sim \text{Dirichlet}(\theta),
% \end{equation} 
% with $\theta \in \R^{p}$ a hyperparameter. Similarly, the topic proportion for document $i$, denoted $ W_{i \cdot} $, is assumed to be sampled from a Dirichlet with hyperparameter $\alpha \in \R^{K}$, with $K$ indicating the number of topics:  
% \begin{equation}\label{eq:dirichlet_samplingW}
%     W_{i \cdot} \sim \text{Dirichlet}(\alpha),\quad \forall i \in [n].
% \end{equation} 
Efforts to incorporate metadata have largely focused on adding additional information at the beginning of this generative model by appropriately modifying the Dirichlet priors. 
%For instance, the Correlated Topic Model approach by \cite{blei2006correlated} assumes a covariance structure on the topic assignments for each word within a document. It proposes generating a topic assignment for each document from a multinomial distribution $\mathrm{Multi}(f(\eta))$, where the covariance between words within a document is parameterized as $\Sigma$ in the prior distribution $\eta \sim N(\mu, \Sigma)$. 
For instance, the dynamic topic modeling approach of \cite{blei2006dynamic} assumes that documents are observed sequentially, and that consecutive documents have similar topic mixture weights. To accommodate this prior, the authors suggest an autoregressive structure on $W$, replacing the Dirichlet sampling in equation \eqref{eq:dirichlet_samplingW} by a sequential sampling mechanism of the form $ W_{i+1} = \text{softmax}(\eta_{i+1})$, with $\eta_{i+1} \sim N(\eta_{i}, \sigma^2 I) .$ \cite{roberts2014structural} extends this approach by using document-level covariates $X_i$, namely $W_{i\cdot} =\text{softmax}(\eta_{i})$, with $\eta_{i} \sim N( X_{i}\beta, \Sigma) .$ 
%and propose modeling correlations between documents by replacing step \ref{eq:dirichlet_samplingW} by a logistic normal sampling step of the form: $W_{i\cdot} =\text{softmax}(\eta_{i})$, with $\eta_{i} \sim N( X_{i}\beta, \Sigma) .$  
By contrast, the work of \cite{mcauliffe2007supervised} incorporates metadata into LDA  by adding a final step to the generating mechanism, explicitly regressing the document-level covariate $y\in \mathbb{R}$ on topic mixture weights: $y \sim N(W_{i\cdot}\eta, \sigma^2)$. 

 While these methods allow the flexible incorporation of additional information to the original LDA framework, the metadata is usually assumed to come as a matrix of additional covariates. These approaches thus need to be appropriately tailored depending on the nature of the covariates considered (e.g. changing the normal prior of \cite{mcauliffe2007supervised} to a Bernouilli or multinomial in the case of categorical covariates, etc). Such changes might introduce additional complexity in the updates, and in cases where certain covariates have no obvious prior, applicability becomes restricted. Most notably, these methods are difficult to adapt to the case where the metadata comes under the form of a graph, which provides a flexible way of encoding complex covariate structures or spatial information. For example, in our corpus of recipes (Section~\ref{sec:experiments:whatscooking}), the origin of recipes is more easily modeled as a graph, rather than a matrix of covariates. Working with a document-similarity graph bypasses the need to adapt the method to different types of covariates, as long as the metadata can be mapped into a similarity metric between two documents.

To the best of our knowledge, the only extension of LDA amenable to the graph setting is that of \cite{chen2020modeling}. There, the authors leverage the presumed similarity between connected documents by regularizing the $\alpha_i$'s in equation \eqref{eq:dirichlet_samplingW} with respect to a known document graph $\mathcal{G}$, so that $\alpha_i \approx \alpha_j$ if documents $i$ and $j$ are connected in the graph.  However, this approach is computationally intensive and, as we find, does not necessarily improve topic accuracy (see Section~\ref{sec:synthetic_experiment}). This LDA-based approach also inherits the limitations of Bayesian methods, such as their potentially slow convergence and lack of theoretical guarantees.

 
\paragraph{Probabilistic Latent Semantic Indexing} Another popular approach to topic modeling is probabilistic Latent Semantic Indexing (pLSI). In a general sense, pLSI can be broadly described as a non-negative matrix factorization technique. In the oracle setting, assuming we have access to the expected frequency matrix $M$, pLSI can be understood as solving a constrained rank $K$ decomposition of the form:
\begin{equation*}
\begin{split}
    \widehat{W}, \widehat{A}  &= \text{argmin}_{W \in \R^{n \times K}, A\in \R^{K \times p}} \| M - WA\|_F^2 \\
    &\text{ such that } \forall i \in [n], \sum_{k=1}^K W_{ik}=1, \quad \forall j \in [p], \sum_{k=1}^K A_{kj}=1
    \end{split}
\end{equation*}


%Denote word as $w_j$ for $j = 1, \cdots, p$, document as $d_i$ for $i=1,\cdots, n$, and topic as $t_k$ for $k=1,\cdots, K$, the probability of observing word $j$ in document $i$ can be decomposed as the inner product of document-topic and topic-word weight.
%In this setting, since $M_{ij}$ corresponds to the expected frequency (or probability) of word $j$ in document $i$, the entries of both $A$ and $W$ can be interpreted as probability distributions using Bayes' formula:

%\begin{equation}\label{eq:totl_prob} 
%\begin{split}
%  M_{ij} &= \P[\text{word } j \mid \text{document } i ] = \sum_{k=1}^{K} \P[\text{word } j \mid \text{Topic } k]\P[\text{Topic } k \mid \text{ document i}) \\
%  &= \sum_{k=1}^{K} A_{kj} W_{ik}\qquad \text{with } A_{kj}=\P[\text{word } j \mid \text{Topic } k], \qquad W_{ik}=\P[\text{Topic } k \mid \text{ document i}) 
%  \end{split}
%\end{equation}

% Denote $\bf M \in \mathbb{R}^{n \times p}$ as the true document-word proportion. Equation~\ref{eq:totl_prob} can be rewritten in  matrix form, $$\bf M = \bf W \bf A$$ where $\bf W \in \mathbb{R}^{n \times K}$ is the document-topic weight matrix and $\bf A \in \mathbb{R}^{K \times p}$ is the topic-word weight matrix with $\sum_{j=1}^{p} W_{ij}=1$ and $\sum_{k=1}^{K} A_{kj}=1$.
% Denote $N_i$ as the length of the $i^{\mathrm{th}}$ document. The observed matrix $\bf X = \left[ X_1^{\top}, X_2^{\top}, \cdots, X_n^{\top} \right]^{\top}\in \mathbb{R}^{n \times p}$ is a noisy version of $\bf\Pi$ where each document's word count vector $N_i X_i \in \mathbb{R}^{p}$ is drawn from a multinomial distribution $N_i X_i \sim \text{Multinomial}(N_i, \Pi_i)$.
% We thus write the observed word-frequency matrix $X$ as:

% \begin{equation}\label{eq:signal_plus_noise}
% \bf X = \bf M + \bf Z = \bf U \bf \Sigma \bf V^{\top} + \bf Z = \bf W \bf A + \bf Z
% \end{equation}


% where $Z$ corresponds to some centered multinomial noise.

% Probabilistic Latent Semantic Index aims to recover the matrices $\A$ and $\W$ respectively. 

pLSI has a rich history in the statistics literature, and offers a robust and scalable alternative to LDA. There has been extensive work on the estimation of topic-word matrix $A$ \citep{ke2017new}. \cite{ke2017new} has established rigorous bounds on the estimation of the topic-word matrix $A$.  For the estimation of document-topic matrix $W$, \cite{klopp2021assigning} exploited the simplex structure of its singular vectors to hunt for $K$ vertices, also endowing their estimates with high-probability upper bounds on $\ell_1$ and $\ell_2$ error. However, as explained in Section~\ref{sec:model}, these methods are not likelihood-based methods and are characterized by a rigid estimation framework, within which the incorporation of covariates or known correlations within the documents is not trivial. Recent work \cite{bing2020optimal, wu2023sparse, tran2023sparse} have just begun considering the addition of more structure to the standard pLSI model, focusing for the most part on leveraging the supposed sparsity of $A$. To the best of our knowledge, the addition of correlation or similarity between documents remains an open question.

